Transfer-based adaptive tree for multimodal sentiment analysis based on user latent aspects

Multimodal sentiment analysis benefits various applications such as human-computer interaction and recommendation systems. It aims to infer the users' bipolar ideas using visual, textual, and acoustic signals. Although researchers affirm the association between cognitive cues and emotional manifestations, most of the current multimodal approaches in sentiment analysis disregard user-specific aspects. To tackle this issue, we devise a novel method to perform multimodal sentiment prediction using cognitive cues, such as personality. Our framework constructs an adaptive tree by hierarchically dividing users and trains the LSTM-based submodels, utilizing an attention-based fusion to transfer cognitive-oriented knowledge within the tree. Subsequently, the framework consumes the conclusive agglomerative knowledge from the adaptive tree to predict final sentiments. We also devise a dynamic dropout method to facilitate data sharing between neighboring nodes, reducing data sparsity. The empirical results on real-world datasets determine that our proposed model for sentiment prediction can surpass trending rivals. Moreover, compared to other ensemble approaches, the proposed transfer-based algorithm can better utilize the latent cognitive cues and foster the prediction outcomes. Based on the given extrinsic and intrinsic analysis results, we note that compared to other theoretical-based techniques, the proposed hierarchical clustering approach can better group the users within the adaptive tree.

==> Sample-Algorithm <==
\begin{algorithm}[H]
			\caption{Stack-Wise Max. Spanning Tree (SW-MST)}
			\label{alg6}
			\textbf{Input:} $G$\\
			\textbf{Output:} $G', S$
			\begin{algorithmic}[1]
				\STATE $\mathbb{N}'=\emptyset, \mathbb{L}'=\emptyset, \mathbb{N}''= \mathbb{N}, \mathbb{L}''= \mathbb{L}, S=\emptyset $
				\WHILE{$\mathbb{L}'' \neq \emptyset$}
				\STATE $l=Min(\mathbb{L}'')$
				\STATE $S.push(l)$
				\STATE $\mathbb{L}''.remove(l)$
				\ENDWHILE
				\WHILE{$\mathbb{N}'' \neq \emptyset$}
				\STATE $\;l=S.pop()$
				\STATE $\;\mathbb{L}'.append(l)$
				\IF{$l[0] \notin \mathbb{N}'$}
				\STATE $\mathbb{N}'.append(l[0])$
				\ENDIF
				\IF{$l[1] \notin \mathbb{N}'$}
				\STATE $\mathbb{N}'.append(l[1])$
				\ENDIF
				\IF{$l[0] \in \mathbb{N}''$}
				\STATE $\mathbb{N}''.remove(l[0])$
				\ENDIF
				\IF{$l[1] \in \mathbb{N}''$}
				\STATE $\mathbb{N}''.remove(l[1])$
				\ENDIF
				\ENDWHILE
				\STATE $G'=(\mathbb{N}',\mathbb{L}')$
				\STATE return $G'$, $Avg(\mathbb{L}')$
			\end{algorithmic}
		\end{algorithm}	
